Construction of Hierarchical Neural Architecture Search Spaces based on Context-free Grammars

The discovery of neural architectures from simple building blocks is a long-standing goal of Neural Architecture Search (NAS). Hierarchical search spaces are a promising step towards this goal but lack a unifying search space design framework and typically only search over some limited aspect of architectures. In this work, we introduce a unifying search space design framework based on context-free grammars that can naturally and compactly generate expressive hierarchical search spaces that are 100s of orders of magnitude larger than common spaces from the literature. By enhancing and using their properties, we effectively enable search over the complete architecture and can foster regularity. Further, we propose an efficient hierarchical kernel design for a Bayesian Optimization search strategy to efficiently search over such huge spaces. We demonstrate the versatility of our search space design framework and show that our search strategy can be superior to existing NAS approaches. Code is available at https://github.com/automl/hierarchical_nas_construction.

==> figures/overview.tex <==
\begin{figure}
    \centering
        \begin{subfigure}[b]{\linewidth}
    \vspace{.3cm}
    \centering
      $\texttt{Sequential}(\texttt{Residual}(\texttt{conv},~\texttt{id},~\texttt{conv}),\; \texttt{Residual}(\texttt{conv},~\texttt{id},~\texttt{conv}),\;\texttt{fc})$
    \caption{Algebraic architecture expression for two residual blocks followed by a linear layer.}
    \label{fig:architecture_example}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
        \centering
         \vspace{.38cm}
        \begin{tikzpicture}
           [->,>=stealth',auto,node distance=0.25cm,
          thick,main node/.style={circle,draw,minimum size=0.1cm}]
    
          \node[main node] (1) at (0,0) {};
          \node[main node] (2) at (2,0) {};
          \node[main node] (3) at (4,0) {};
          \node[main node] (4) at (6,0) {};
          \node[main node] (5) at (8,0) {};
          \node[main node] (6) at (10,0) {};
        
          \path[every node/.style={font=\sffamily\small}]
            (1) edge node [] {\texttt{conv}} (2)
            (2) edge node [] {\texttt{conv}} (3)
            (1) edge[bend left] node [] {\texttt{id}} (3)
            (3) edge node [] {\texttt{conv}} (4)
            (4) edge node [] {\texttt{conv}} (5)
            (3) edge[bend left] node [] {\texttt{id}} (5)
            (5) edge node [] {\texttt{fc}} (6);
        \end{tikzpicture}
        \caption{Computational graph corresponding to (a).}
        \label{fig:architecture_example}
    \end{subfigure}
     \begin{subfigure}[b]{\linewidth}
     \vspace{.38cm}
        \centering
        \begin{tikzpicture}
           [->,>=stealth',auto,node distance=0.25cm,
          thick,main node/.style={circle,draw,minimum size=0.1cm},op node/.style={rectangle,draw=white,minimum size=0.1cm}]
    
          \node[main node] (1) at (0,0) {};
          \node[main node] (2) at (4,0) {};
          \node[main node] (3) at (8,0) {};
          \node[main node] (4) at (10,0) {};
          \node[draw=white] at (6,0.3) {\texttt{Sequential}($\cdot$, $\cdot$, $\cdot$)};
          
          \node[main node] (5) at (-1, -2) {};
          \node[main node] (6) at (1, -2) {};
          \node[main node] (7) at (3, -2) {};
          \node[draw=white] at (1,-1.2) {\texttt{Residual}($\cdot$, $\cdot$, $\cdot$)};
          
          \node[draw=white] (12) at (-0.5,-3) {\texttt{conv}};
          \node[draw=white] (13) at (1,-3) {\texttt{id}};
          \node[draw=white] (14) at (2.5,-3) {\texttt{conv}};
          
          \node[main node] (8) at (4, -2) {};
          \node[main node] (9) at (6, -2) {};
          \node[main node] (10) at (8, -2) {};
          \node[draw=white] at (6,-1.2) {\texttt{Residual}($\cdot$, $\cdot$, $\cdot$)};
          
          \node[draw=white] (15) at (4.5,-3) {\texttt{conv}};
          \node[draw=white] (16) at (6,-3) {\texttt{id}};
          \node[draw=white] (17) at (7.5,-3) {\texttt{conv}};
          
          \node[op node] (11) at (9.5,-1.2) {\texttt{fc}};
          
          \node[op node, blue] (18) at (12,0) {Level 1};
          \node[op node, blue] (19) at (12,-1.6) {Level 2};
          \node[op node, blue] (20) at (12,-3) {Level 3};
        
          \path[every node/.style={font=\sffamily\small}]
            (1) edge node [] {} (2)
            (2) edge node [] {} (3)
            (3) edge node [] {} (4)
            
            (5) edge node [] {} (6)
            (6) edge node [] {} (7)
            (5) edge[bend left] node [] {} (7)
            
            (8) edge node [] {} (9)
            (9) edge node [] {} (10)
            (8) edge[bend left] node [] {} (10)
            
            (2,-0.2) edge[blue, dashed] node [] {} (1.1,-1)
            (6,-0.2) edge[blue, dashed] node [] {} (6,-1)
            (9,-0.2) edge[blue, dashed] node [] {} (11.north)
            
            (0,-2.2) edge[blue, dashed] node [] {} (12.north)
            (1,-1.5) edge[blue, dashed] node [] {} (13.north)
            (2,-2.2) edge[blue, dashed] node [] {} (14.north)
            
            (5,-2.2) edge[blue, dashed] node [] {} (15.north)
            (6,-1.5) edge[blue, dashed] node [] {} (16.north)
            (7,-2.2) edge[blue, dashed] node [] {} (17.north);
        \end{tikzpicture}
        \caption{Algebraic decomposition into other algebraic expressions, \ie, graph operators or primitive computations.}
        \label{fig:architecture_hierarchical}
    \end{subfigure}
    \caption{We represent neural architectures as algebraic expressions (a) which represent the (edge-attributed) computational graph (b). These algebraic expression are hierarchically composed of other algebraic expressions out of graph operators (\eg, \texttt{Residual}($\cdot$, $\cdot$, $\cdot$)) or primitive computations (\eg, conv) (c).}
\end{figure}
